Using Alloy to Formally Model and Reason About an OpenFlow Network Switch

Openflow provides a standard interface for separating a network into a data plane and a programmatic control plane. This enables easy network reconfiguration, but introduces the potential for programming bugs to cause network effects. To study OpenFlow switch behavior, we used Alloy to create a software abstraction describing the internal state of a network and its OpenFlow switches. This work is an attempt to model the static and dynamic behaviour a network built using OpenFlow switches.

==> commands.tex <==
\newcommand{\codeFont}[1]{\textcolor[rgb]{0,0,1}{\textbf{#1}}}
\newcommand{\myVerbatim}[1]{
\begin{Verbatim}
#1
\end{Verbatim}
}


==> implementation.tex <==
\subsection{Alloy language}
"Alloy is a language for describing structures and a tool for exploring them. It has been used in a wide range of applications from finding holes in security mechanisms to designing telephone switching networks. The Alloy language is a simple but expressive logic based on the notion of relations." \cite{alloylang}
\subsection{Alloy model}
An Alloy model is a collection of constraints that describes (implicitly) a set of structures. In this section, we will show implementation of OpenFlow switch in Alloy.
Keyword "sig" is used to define sets. For example \textbf{one sig Network{content:some Node}} defines there is exactly one network which includes a set of nodes(one or more) which is called content. This is a simple model(detailed are removed from actual code to make it more comprehensive) which includes all the required sets(entities in network). Controller or Switch extend Node, in which each Node has some ports. Each Switch has at least one Table and a buffmsg which is a buffer keeping all in and out messages.Each Table has some FlowEntry. Each entry contains a MatchFiled, a Counter and the corresponding Action. When a packet arrives at the Switch, it is compared with entries in the flow table. If packet is matched with one of the entries, the entry's counter is increased and associated action will be executed(for example forward to a specific port, drop the packet). The most important rules for matching are packet's source IP, packet's destination IP, and incoming port(the port in which) which are considered in our model. If no match is found in a flow table, the outcome depends on switch configuration: the packet may be forwarded to the controller over the OpenFlow channel, dropped, or may continue to the next flow table.

The model corresponding to the code is shown in  Figure~\ref{fig:model1}(unnecessary details are removed). As you see there are a few inconsistency in the model. For example port3 is connected to itself, in the real network a switch's port is connected to  port of another switch or controller. The other problem is root table's next table pointer is pointing to itself. Also root table is next table for both itself and table0. Thus just defining the model itself is not enough and we have define properties of desired model. To achieve this, we have define facts to enforce Alloy to just give us the models satisfying facts. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Tables}

In order to impose each table is only next table of at most one table(no same next table for two different tables), we used the following fact:


To impose root is not the next table of any table:

To impose next table of no table can be the table itself

Imposing these facts, we got the following model in ~\ref{fig:model5}. 

As you can see, table's next table point to root table, which is not valid. The reason is th following, we just mentioned for all the tables in switch next table cannot be root table. But here table does not belong to any switch. So we have to add another fact: 

To impose all the tables should belong to one switch:

Thus we will impose the following fact which implies every port belongs to exactly one node:

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Some other facts about tables are listed in below:
////


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Ports}
To eliminate inconsistency problem in port(in case port 3 is connected to itself in ~\ref{fig:model1}), the following fact is added to the code:
// //
This prevents not only a port cannot be connected to itself, but also it cannot be connected to a port in the same node(switch/controller).
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

There are some other facts about port which need to be considered. These facts are:
// //
\subsection{Flow entries}


To impose every flow entry is contained in only one table:
// //
There are more facts which are not discussed here, and you can see them in the code.


After adding required facts, the model will be a valid model which corresponds to real network. The model is shown in ~\ref{fig:model2}
We have a model which shows the static state of network. Now we want to have a dynamic model and observe effect of each event on the network's state.
\begin{verbatim}

\end{verbatim}


